The Einstein Probe Mission

The Einstein Probe (EP) is a mission designed to monitor the sky in the soft X-ray band. It will perform systematic surveys and characterisation of high-energy transients and monitoring of variable objects at unprecedented sensitivity and monitoring cadences. It has a large instantaneous field-of-view (3,600 sq. deg.), that is realised via the lobster-eye micro-pore X-ray focusing optics. EP also carries a conventional X-ray focusing telescope with a larger effective area to perform followup observations and precise positioning of newly-discovered transients. Alerts for transient objects will be issued publicly and timely. The scientific goals of EP are concerned with discovering faint, distant or rare types of high-energy transients and variable sources. Within the confines of a modest-sized mission, EP will cover a wide range of scientific topics, from the nearby to high-redshift Universe. The Einstein Probe is a mission of the Chinese Academy of Sciences, and also an international collaborative project. This paper presents the background, scientific objectives, and the mission design including the micro-pore optics and CMOS technologies adopted, the instruments and their expected performance, and the mission profile. The development status of the project is also presented.

==> ep-cmos.tex <==
%
\subsection{CMOS detectors}

{\it
Suggested length: 1-2 page\\

This subsection is to be provided by Zhixing. \\

introduce CMOS detectors used for WXT\\
present some of the basic performance and test results of the CMOS for WXT (some results from the recent paper by Wu et al. can be used\\
summarising the performance and conclusion that the CMOS sensor can satisfy the requirement of EP WXT \\
A few useful figures can be provided
}

Complementary Metal-Oxide-Semiconductor (CMOS) sensor has been widely used during the last decade in industrial and consumer electronics. Thanks to the rapid development of semiconductor manufacturing, the performance of CMOS sensor have been raised significantly. Several designers have developed many scientific CMOS sensor products. Unlike the traditional Charged Coupled Device (CCD) detector, the CMOS sensor could be manufactured by the standard CMOS semiconductor process worldwide. The pixel of the CMOS sensor consists of several transistors (typically 4T) to realize the transfer, reset, row selection, and source follower readout. Only one row is switched on when the readout works. An amplifier and an Analog to Digital Converter (ADC) are placed in each column to realize the readout of the whole row signal simultaneously. This readout structure makes the read out speed of the CMOS sensor quite fast.

Compared to the CCD detector, the apparent advantages of CMOS sensors are that there is no charge transfer and the faster read out speed of the whole array. Usually, CCD devices must have a perfect charge transfer efficiency to guarantee no loss of the initial electrons after many transfers (even several thousands of transfers). This characteristic makes the CCD detectors significant degradation after radiation. Because only one row is switched on, there is no transfer during the read out of the signal. Therefore, the CMOS sensor is a better choice for use in a radiation environment, especially in space orbit or harsh radiation conditions. Because the number of ADC channels increased in several orders of magnitude, the read out time of a single frame of the CMOS sensor can be reduced to several mini seconds. This high speed lowers the cooling system's requirement, of which is needed to decrease the influence of dark current. The upper limit count rate for single photon detection is promoted in two or three orders of magnitude. Besides those advantages, the cost of the CMOS sensor is lower than the CCD sensor either. The complexity of the readout electronics is reduced because most of the digital electronics are integrated inside the CMOS sensor. Besides those advantages, CMOS sensors also have some disadvantages. The dark current nonuniformity is larger than the CCD detector. This phenomenon is quite severe in long time exposure usage. The photon response nonuniformity must also be considered carefully because of the difference of the amplifiers from pixels to pixels.

For the application of X-ray astronomy, the back illuminated CMOS sensor is needed because of the short penetration length for soft X-ray photons. We customized a large format back illuminated CMOS sensor in 2017 and got the final product in 2019. The image of this customized CMOS sensor is shown in Figure \ref{cmos_photo}. The parameters are summarized in Table \ref{table_cmos}. The pixel size is designed larger than the former products to meet the requirement for X-ray detection. The read out noise is lower than 5 elections in the frame rate of 20 Hz. As shown in Figure \ref{fespec}, the energy resolution is 210 eV at room temperature for the $K\alpha$ emission line of Fe55 source. The detail of the performance of this customized CMOS sensor could be found in Wu et al. 2022 \cite{wu2022}.
Several optimizations of the CMOS sensor have been made in the last few years for usage in X-ray detection, including the customization of our large format large pixel product. The entrance window of the sensor had been minimized to several nanometers to increase the quantum efficiency of low energy X-ray photons. The epitaxial layer depth and the depletion depth have been raised to enlarge the quantum efficiency for the higher energy region.
The technology of CMOS sensors is developing very rapidly. A size of 9 cm $\times$ 9 cm product has been manufactured while writing this handbook. Another fascinating feature of the CMOS sensor is that the on-chip function could be customized according to the application. For example, Gao et al. 2021 designed an on-chip event detection algorithm inside the CMOS sensor, of which achieve a frame rate of 8000 Hz for electron detections\cite{gao2021}.

Besides the CMOS sensor discussed above, another sort of CMOS sensor is the hybrid CMOS sensor. Different photodiode material could be used according to the response wavelength. The signal is read by the underneath readout integrated circuit for hybrid CMOS sensor. The Lynx X-ray surveyor mission is planning to use hybrid CMOS detector as the focal plane detector\cite{hull2019}.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{cmos.png}
\caption{Figure of CMOS sensor.}
\label{cmos_photo}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{ l | l }
\hline
Image area & $6\ \rm{cm}\times 6\ \rm{cm}$ \\ \hline
Pixel size & $15\ \rm{\mu m}\times 15\ \rm{\mu m}$ \\ \hline
Epitaxial thickness & $10\ \rm{\mu m}$ \\ \hline
%Total pixels & $4154\times 4112$ \\ \hline
Number of pixels & $4096\times 4096$ \\ \hline
Frame rate & 20 fps (maximum 100 fps)\\ \hline
Readout noise & $\rm{< 5.0\ e^-}$ at high gain\\ \hline
Dark current & $\rm{< 0.02\ e^-/pixel/s\  @\ -30^{\circ}\!C}$ \\
& $\rm{< 10\ e^-/pixel/s\  @\  20^{\circ}\!C}$ \\ \hline
Energy resulotion & $210\ eV@5.9 keV$\\ \hline
Full well capicity & 120 $ke^-$ \\ \hline
Power & 1.6 W \\ \hline
\end{tabular}
\caption{Basic properties of the customized CMOS detectors.}
\label{table_cmos}
\end{table}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{fespec.pdf}
\caption{Spectrum of Fe55 source with the customized CMOS sensor.}
\label{fespec}
\end{figure}


==> ep-con.tex <==

\section{Conclusion}
\label{sec:con}

The Einstein Probe is a mission of the Chinese Academy of Sciences (CAS) dedicated to time-domain high-energy astrophysics. 
The primary science objectives are: (1) Discover and characterise cosmic X-ray transients, particularly faint, distant and rare X-ray transients, in large numbers. (2) Discover and characterise X-ray outbursts from otherwise normally dormant black holes.  (3) Search for X-ray sources associated with gravitational-wave events and precisely locate them. These populations of cosmic high-energy transients will be characterised over wide time-scales and at high cadences, revealing new insights into a diverse set of systems including dormant black holes, neutron stars, supernova shock breakouts, active galactic nuclei, X-ray binaries, gamma-ray bursts, stellar coronal activity, and electromagnetic-wave sources and gravitational-wave events. Meanwhile, EP will also monitor the variability of various types of X-ray sources in large samples all over the sky. In light of the multi-messenger and multi-wavelength all-sky monitoring capability highly anticipated in the next decade, EP will produce a legacy data set in the X-ray band that are key to characterising and understanding the nature of cosmic transients and variables, by working in synergy with the sky surveys by other facilities. 

The mission will address some of the key questions in astrophysics and cosmology, and details of the physics which operates in extreme conditions of strong gravity. These include the prevalence of massive black holes in the Universe and how they formed and evolved; how black holes accrete mass and launch jets; the astrophysical origins and underlying processes of gravitational wave events; the progenitors and processes of supernovae; when and where did the first stars form in the early Universe and how they re-ionize the Universe.

EP employs a very large instantaneous field-of-view (3600 square degrees), along with moderate spatial resolution (FWHM ~5 arcmin) and energy resolution.  
Its wide-field imaging capability is achieved by using established technology of novel lobster-eye optics, thereby offering unprecedentedly high sensitivity and large Grasp, which would supersede previous and existing X-ray all-sky monitors. 
EP also carries a conventional X-ray focusing telescope with a larger effective area to perform follow-up characterization and precise localization of newly-discovered transients. 
Public transient alerts will be issued rapidly to trigger multi-wavelength follow-up observations from the world-wide community. 
Over three orbits almost the entire night sky will be sampled, with cadences ranging from several to a few ten revisits per day. 
The mission is aimed for launch by end 2023 with a nominal lifetime of 3 years, and 5 years as a goal.

The wide, deep and fast time-domain surveys of EP will result in breakthroughs that may have profound impact in a broad range of fields in astrophysics, and will produce an invaluable database with long-lasting benefit for future time-domain surveys and research.






==> ep-mpo.tex <==
%
\subsection{Lobster-eye micro-pore optics}
\label{sec:mpo}

X-ray photons, having energies a thousand times that of optical photons, can go right through the surfaces of all substances unaffected.
Generally, their directions can be barely changed by very smooth surface. However, when the incidence angle is small enough relative to the surface (not to the surface normal),
the well-know grazing incidence reflections occur. In order to obtain enough effective area, lots of reflection surfaces have to be nested and configured in a certain way.
A conventional configuration is the Wolter-I optics, which contains nested parabolic surfaces followed by hyperbolic surfaces.
This kind of optics is rotationally symmetric, which naturally forms an optical axis. In General, the incidence angle to the optical axis get larger, the imaging qualification get worse. As a result, the FoV of Wolter-I optics is quite small, typically less than one degree.



Alternatively, the Lobster-eye Micro-Pore Optics (MPO) (Angel,J.R.P.1979) \cite{angel1979}, which has the similar imaging principle with the eyes of lobsters, can reach an unrestricted FoV.
The lobster-eye optics is made of a thin spherical plate with millions of square micro-pores nesting in it \ref{fig:secmpo_photo}. The axes of all pores point radially to the curvature centre of the spherical plate, and the adjacent walls of pores are orthogonal to each other. As shown in figure \ref{fig:mpo_principle}, incoming X rays at a grazing incidence angle is reflected off the walls of the tiny pores, and is redirected onto a focal spherical plate with a radius of half the curvature of the optics. Such a focusing optics produces a cruciform imaging (Zhao et~al.2017)\cite{zhao2017}, as shown in Figure \ref{fig:mpo_psf}, consisting of a central peaking spot produced by two reflections from adjacent walls of the tiny pores and two cross-arms produced by single reflections.
On the ideal lobster-eye optics, a same large number of pores take part in the reflections for any given direction of incoming light.
In another word, this kind of configuration has no preferential optical axis, and can thus get an un-vignetted FoV as large as the entire solid angle of $4\pi$ in principle, which provides a unique technique for wide-field X-ray imaging.

For the currently commercially available MPO pieces, a large focusing gain of $\sim$2000 and a moderate resolution of arc-minutes can be achieved.
In practice, the Wide-field X-ray Telescope (WXT) aboard Einstein Probe satellite just adopts the Lobster-eye optics, which obtains a FoV of thousands of square degrees with very light weight. you can find more details in the section about WXT.



 \begin{figure}
    \includegraphics[width=0.5\textwidth]{fig_secmpo_photo.pdf}
    \caption{The photo of a MPO chip without optical block filter (left) and pore structures under microscope.}
    \label{fig:secmpo_photo}
\end{figure}



 \begin{figure}
    \includegraphics[width=0.5\textwidth]{PrincipleMPO.pdf}
    \caption{The imaging principle of Lobster-eye Micro-Pore Optics.}
    \label{fig:mpo_principle}
\end{figure}



 \begin{figure}
    \includegraphics[width=0.5\textwidth]{MPO_PSF.pdf}
    \caption{The PSF of a Lobster-eye Micro-Pore Optics by simulations.}
    \label{fig:mpo_psf}
\end{figure}


{\it 
This subsection is to be provided by Chen Zhang. Suggested length: 1-2 page

introduce MPO and its imaging principle \\
present some of the basic properties of MPO imaging, both simulation and test results, PSF, etc. previous publications of our team can be referred to \\
A few useful figures can be provided, suggest to include (at least) the MPO imaging principle, simulated PSF \\
Below is the text for this part from my previous proceedings paper on EP at the MAXI conference. It can be used as a reference, and can provide a basis for expansion and updates.\\
}


In general, X-ray focusing is realised by multiple grazing incidence reflections on surfaces 
almost parallel to the direction of incident X-rays. 
The conventionally and commonly adopted configuration is the Wolter-I optics, 
which reflects X-rays by a tubular, rotationally symmetric parabolic surface 
followed by a hyperbolic surface. 
The FoV of such optics is inherently small, typically less than one degree.
Alternatively, the Lobster-eye Micro-Pore Optics (MPO) \cite{angel79},    
which mimics the imaging principle of the eyes of lobsters (Figure \ref{fig:lobster_eye}),
can reach an unrestricted FoV.
The  lobster-eye optics is made of a thin spherical micro-channel plate with millions of 
square micro-pores, the axes of which all point radially to a common centre of curvature. 
Incoming light at a grazing incidence angle is reflected off the walls of the many tiny pores, 
and is brought onto a focal sphere with a radius of half the curvature of the optics.
For any given direction of incoming light,  a same large number of pores, 
whose reflection surfaces are configured orthogonal to each other, 
take part in the reflection.  
Such a configuration has no preferential optical axis, and can thus deliver an un-vignetted 
FoV as large as, in principle,  the entire solid angle of $4\pi$.  

Such a focusing optics produces true imaging with a cruciform
point spread function, which has a central peaking spot 
produced by two reflections from adjacent walls of the pores and 
cross-arms produced by single reflections. 
It can yield a large focusing gain of $\sim$2000, 
and a moderate resolution of FWHM the order of arc-minutes  delivered by 
the currently commercially available MPO pieces.
In practice, the MPO Lobster-eye optics can achieve a FoV 
of thousands of square degrees with very light weight,  
which is unique for wide-field X-ray imaging.
Figure\,\ref{fig:mpo-prototype} shows a demonstration prototype of a portion
of the optics assembly of one WXT module (left panel),
 as well as an X-ray image obtained at the focal plane for a point-like
X-ray source, i.e. PSF (right panel).



==> ep-wxt-wmy-template.tex <==
\subsection{Wide-field X-ray Telescope} 

\subsubsection{WXT optics and performance}

%Design of WXT, including description of the components and specifications \\suggested figures (not limited to): design layout of one wxt module, focal plane detector (CMOS array), picture of one completed QM module \\Previous publications of our team can be cited.

The detection bandpass of WXT is designed as 0.5--4.0\,keV nominally.
To achieve both wide FoV and X-ray focusing in this soft X-ray band, lobster-eye micro-pore optics is adopted for WXT.
WXT consists of 12 identical modules and makes a total vignetting-free FoV of $\sim 3600$ square degrees ($\sim$1.1\,steradian).
Figure\,\ref{fig:wxt-module} shows the layout of one WXT module, which mainly includes lobster-eye optics, detectors and the electronics unit, thermal control system and supporting structures. An optical baffle is setup at the front end of the MPO assembly to shield the stray light from the Sun, the Moon and the Earth.
The optics of each module is composed of $6\times6$ MPO plates with a 375\,mm focal length and a 2.5 \,mm thickness.
A permanent magnet diverter (Wang et~al.2020) \cite{wang2020}, which is comprised of 16 rectangular NdFeB blocks mounted in a square frame to produce a circular magnetic field, is just mounted below the optics in each WXT module to reduce low-energy electrons reaching the detector.
More design parameters of WXT can be found in Table \ref{tab:wxt}.

% can effectively reduce the electron background level of WXT by one order of magnitude.
%One WXT module weights 17\,kg including the MPO mirror assembly, detector and electronics unit, optical baffle, structure and thermal control.

\begin{figure}[]
%\sidecaption[t]
\includegraphics[width=0.5\textwidth]{wxt-module-2.pdf}
\caption{Design of one module of the Wide-field X-ray Telescope aboard Einstein Probe satellite.}
\label{fig:wxt-module}
\end{figure}




%Predicted Instrument performance , some simulated properties, PSF, effective area, theoretical Grasp, background simulations, sensitivity, etc. Previous publications of our team can be cited. Suggest to include briefly an introduction to the QM test and calibration.\\


\begin{table}
\begin{center}
\caption{Main design parameters of WXT.}
\label{tab:wxt}
%\small
\begin{tabular}{|c|c|}
\hline
Specification &  value \\
\hline
Number of modules & 12 \\
\hline
Field-of-view & 3600 sq.deg.  \\
\hline
Focal length  & 375 mm \\
\hline
Spatial resolution fwhm & 5' \\
\hline
Bandpass (keV) & 0.5--4.0 \\
\hline
E resolution @1\,keV & 170 eV   \\
\hline
Effective area @1\,keV &  $\sim$3 cm$^2$ \\
\hline
One Module Mass  & 17\,kg  \\
\hline
\end{tabular}
\end{center}
\end{table}
	


Based on the realistic ray-tracing simulations taking into account the imperfectness of the MPO arrays (Zhao et~al.2014, Zhao et~al.2017) \cite{zhao14}\cite{zhao17}, the effective area curves of WXT are derived as shown Figure\,\ref{fig:wxt-area}, $\sim$3 $\sim$3 at 1 keV. Even thought the effective area for a given direction is not so high, it has nearly the same value across almost the entire FoV, achieving a very large Grasp (effective area times FoV) of $\sim10^4$\,cm$^2$\,sq.deg., which is the largest among all focusing instruments in X-ray band as shown in Figure \,\ref{fig:wxt-grasp}.



\begin{figure}[]
%\sidecaption[t]
\includegraphics[width=0.5\textwidth]{EffArea_WXT.pdf}
\caption{The effective area curves of WXT.}
\label{fig:wxt-area}
\end{figure}




\begin{figure}[]
%\sidecaption[t]
\includegraphics[width=0.5\textwidth]{WXT_Grasp.pdf}
\caption{Comparison of the grasp of WXT with other X-ray focusing instruments (update based on the results in paper\cite{zhao14}).}
\label{fig:wxt-grasp}
\end{figure}


Limited by the current manufacture technology of the MPO plate and the process of assembling, the angular resolution of WXT is $\sim$5\,arcmin (FWHM) for the central focal spot. Based on simulations of the background on the detector caused by X rays (both the cosmic X-ray background and Galactic diffuse emission) and cosmic particles (electrons,positrons,protons and so on) (Zhao et~al.2018) \cite{zhao2018}, we estimate WXT's detecting sensitivity for a point-like source\footnote{Assuming a power law spectrum with a photon index of -2 and a Galactic absorption column  $3\times10^{20}$\,cm$^{-2}$.} to be approximately $\sim1\times10^{-11}$\,ergs\,s$^{-1}$\,cm$^{-2}$ (in the 0.5-4\,keV band) or $\sim$0.3\,mCrab at a exposure time of 1000\,seconds. The result shows that WXT is much more sensitive than previous and current wide-field X-ray monitors, including MAXI and Swift/BAT.


A qualification module of WXT has been calibrated with X-ray beams, which presents a good agreement of experimental results with simulation ones. A symmetrical image of WXT under the parallel X-ray beam of Cu-L is shown in Figure\,\ref{fig:wxt-PSF}, while an angular resolution of better than 5 arcmin is obtained for some certain incidence directions.


\begin{figure}[]
%\sidecaption[t]
\includegraphics[width=0.5\textwidth]{WXT_PSF_Test.pdf}
\caption{One true image of WXT in calibration experiment with X-ray beam of Cu-L. The palette presents log scale.}
\label{fig:wxt-PSF}
\end{figure}



\begin{figure}[]
%\sidecaption[t]
\includegraphics[width=0.7\textwidth]{WXT_FWHM.pdf}
\caption{FWHM of WXT by fitting PSF on (right) X and (left) Y dimension in calibration experiment with X-ray beam of Cu-L.}
\label{fig:wxt-FWHM}
\end{figure}







%\subsubsection{Design of WXT}

Design of WXT, including description of the components and specifications \\
suggested figures (not limited to): design layout of one wxt module, focal plane detector (CMOS array), picture of one completed QM module \\
Previous publications of our team can be cited.

\subsubsection{WXT performance}

Predicted Instrument performance , some simulated properties, PSF, effective area, theoretical Grasp, background simulations, sensitivity, etc. Previous publications of our team can be cited.
Suggest to include briefly an introduction to the QM test and calibration.\\

{\it 
Below is the text for this part from my previous proceedings paper on EP at the MAXI conference. It can be used as a reference, and can provide a basis for expansion and update.}\\

To achieve both wide FoV and X-ray focusing, the novel micro-pore optics
in the lobster-eye configuration (see above) is adopted for WXT. 
WXT consists of 12 identical modules with a 375\,mm focal length,
each of which is composed of $6\times6$ mosaicking MPO plates, 
subtending $\sim300$ square degrees.
Figure\,\ref{fig:wxt-module} (upper panel) shows the layout of one WXT module. 
An optical baffle is attached at the front end of the MPO assembly 
to shield optical stray light from the Sun, the Moon and the Earth. 
The 12 modules make a total vignetting-free FoV of WXT of $\sim 3600$ 
square degrees ($\sim$1.1\,steradian),
as  illustrated in Figure\,\ref{fig:wxt-module} (lower panel).

\begin{figure}[]
%\sidecaption[t]
% Use the relevant command for your figure-insertion program
% to insert the figure file.
% For example, with the option graphics use
\includegraphics[width=0.44\textwidth]{wxt-module-design}
\includegraphics[width=0.55\textwidth]{wxt-module-1}
%\includegraphics[scale=.69]{wxt-module-design}
%\includegraphics[scale=.49]{wxt-module-1}
%
% If no graphics program available, insert a blank space i.e. use
%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%
\caption{Design of one module of the Wide-field X-ray Telescope.}
%If the width of the figure is less than 7.8 cm use the \texttt{sidecapion} command to flush the caption on the left side of the page. If the figure is positioned at the top of the page, align the sidecaption with the top of the figure -- to achieve this you simply need to use the optional argument \texttt{[t]} with the \texttt{sidecaption} command}
\label{fig:wxt-module}       % Give a unique label
\end{figure}

WXT has a large-format focal plane of approximately $420$\,mm$\times$420\,mm.
The baseline choice of the focal plane detectors is CMOS imaging sensors, developed at the Gpixel Inc.\ in China.
The current design is to mosaic the focal plane detector of one WXT module by 2x2 CMOS sensors.
This new type of detectors, which are currently being under development,  
have 4\,k$\times$4\,k pixels (of pixel size 15\,micro) and 6\,cm$\times6$\,cm in size. 
The CMOS detectors have some advantages over CCDs for their fast readout speed, 
as fast as several tens of frames per seconds. 
They can thus be operated at moderately low temperatures.
%, $-20^{\circ}$\,C for WXT in the current design.
One WXT module weights 17\,kg including the MPO mirror assembly, detector and electronics unit, 
optical baffle, structure and thermal control.

\begin{table}[]
%\begin{center}
\caption{Specification of WXT}
\label{tab:wxt}     
%\begin{tabular}{ll}
\begin{tabular}{p{5cm}p{3cm}}
\hline\noalign{\smallskip}
Specification &  value \\
\noalign{\smallskip}\svhline\noalign{\smallskip}
Number of modules & 12 \\
Field-of-view & 3600 sq.deg.  \\   
Focal length (mm) & 375 \\
Spatial resolution fwhm & 5' \\
Bandpass (keV) & 0.5--4.0 \\
E resolution (eV) @1\,keV & 170   \\
Effective area @1\,keV (cm$^2$)&  $\sim$3  \\ 
\noalign{\smallskip}\hline\noalign{\smallskip} 
\end{tabular}\\
$^a$ Table foot note (with superscript)
%\end{center}
\end{table}

The nominal detection bandpass of WXT is 0.5--4.0\,keV. 
Figure\,\ref{fig:effarea} shows the effective area curves of WXT  
derived via realistic ray-tracing simulations taking into account the imperfectness
of the MPO arrays \cite{zhao14}. 
The focal plane detector is a CMOS sensor coated with 200\,nm-thick Aluminum.     
The peak effective area is  $\sim$3\,cm$^2$ at around $\sim$1\,keV 
for almost any direction within the FoV except at the edge of the MPO plates.
Thought the effective area for a given direction is not high, it has nearly the same value
across the entire FoV, yielding a very large  Grasp (effective area times FoV) 
of the order of $\sim10^4$\,cm$^2$\,sq.deg., 
which is the largest among all focusing instruments in X-rays. 
Based on simulations of the X-ray background on the detector, including particle background and
incident diffuse X-ray emission (both the cosmic X-ray background and Galactic diffuse emission),
we estimate a detecting sensitivity for a point-like source\footnote{
Assuming a power law spectrum with a photon index of -2 and 
a Galactic absorption column  $3\times10^{20}$\,cm$^{-2}$.} 
for WXT to be approximately
$\sim1\times10^{-11}$\,ergs\,s$^{-1}$\,cm$^{-2}$ (in the 0.5-4\,keV band) 
or $\sim$0.3\,mCrab at 1000\,second exposure\footnote{
It should be noted, however, that these values are based on the simulations
and may be considered to be nominal;
the true sensitivity may be somewhat lower considering possible degradation of 
the performance of the actual MPO plates used, as well as the actual environment of
charged particles in orbit. }, 
much more sensitive than 
previous and current wide-field X-ray monitors, including MAXI and Swift/BAT.   
The angular resolution is $\sim$5\,arcmin  (FWHM) for the central focal spot,
limited by the manufacturing precision of the MPO plates for the current technology,
and possibly by misalignment and distortion of the plates introduced in the process of assembling. 


==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

